Resource allocation problems with expensive function evaluations

The resource allocation problem is among the classical problems in operations research, and has been studied extensively for decades. However, current solution approaches are not able to efficiently handle problems with expensive function evaluations, which can occur in a variety of applications. We study the integer resource allocation problem with expensive function evaluations, for both convex and non-convex separable cost functions. We present several solution methods, both heuristics and exact methods, that aim to limit the number of function evaluations. The methods are compared in numerical experiments using both randomly generated instances and instances from two resource allocation problems occurring in radiation therapy planning. Results show that the presented solution methods compare favorably against existing derivative free optimization solvers.

==> tex/1-Opt_code.tex <==
\Cref{alg: 1-Opt} provides the pseudocode of the 1-Opt method.

\begin{algorithm}[H]
\small
\Begin{
Set $t=0$, set $V^0$ according to initial information, and determine $l^0$\;
Solve $P(f)$ restricted to evaluated data points\;
Denote the solution by $\bm{x}^0$\;
Let $S^{-} = \{i :  x_i^0 >0 \}$ and determine $\theta_i^0$ for all $i\in S^{-}$\;
Let $S^{+} = \{j :  x_j^0 < b_j\}$ and determine $\eta_j^0$ for all $j\in S^{+}$\;
Set $d^0 = \max \{\eta_j^0  - \theta_i^0~|~i \in S^{-},j\in S^{+}, i\neq j\}$\;
\While{$d^t > 0$}{
\For{$i=1:n$}{
	\uIf{$i \in S^{+} \land v_{i,x_i^t+1}^t=0$}{
	$\Delta_i^{+,t} = \eta_i^t - \min_j \{\theta_j^t :j \in S^{-}\backslash\{i\},~ v_{j,x_j^t-1}^t=1\}$\;}
	\Else{$\Delta_i^{+,t} = -\infty$\;}
	\uIf{$i \in S^{-} \land v_{i,x_i^t-1}^t=0$}{
	$\Delta_i^{-,t} = \max_j \{\eta_j^t : j \in S^{+}\backslash\{i\} ,~ v_{j,x_j^t+1}^t=1\} - \theta_i^t$\;}	
	\Else{$\Delta_i^{-,t} = -\infty$\;}
}	
Set $i_t = \argmax_i \max\{\Delta_i^{-,t}, \Delta_i^{+,t} \}$\;
\uIf{$\Delta_{i_t}^{-,t} < \Delta_{i_t}^{+,t}$}{
Set $\lambda_t = 1$ and let $j_t = \argmin_j \{\theta_j^t :j \in S^{-}\backslash\{i_t\},~ v_{j,x_j^t-1}^t=1\}$\;
}\Else{
Set $\lambda_t = -1$ and let $j_t = \argmax_j \{\eta_j^t : j \in S^{+}\backslash\{i_t\} ,~ v_{j,x_j^t+1}^t=1\}$\;
}
Set $V^{t+1} = V^t$\;
Evaluate $f_{i_t}(x_{i_t}^t+\lambda_t)$ and set $v_{i,x_{i_t}^t+\lambda_t}^{t+1}=1$\;
Solve $P(f)$ restricted to evaluated data points\;
Denote the solution by $\bm{x}^{t+1}$\;
Determine $l^{t+1}$\;
Let $S^{-} = \{i :  x_i^{t+1} >0 \}$ and determine $\theta_i$ for all $i\in S^{-}$\;
Let $S^{+} = \{j :  x_j^{t+1} < b_j\}$ and determine $\eta_j$ for all $j\in S^{+}$\;
Set $d^t = \max \{\eta_j^t  - \theta_i^t~|~i \in S^{-},j\in S^{+}, i\neq j\}$\;
Set $t \leftarrow t+1$\;
}
Set $\bm{x}^{\text{1-opt}} = \bm{x}^{t}$\;
}
\caption{1-Opt method \label{alg: 1-Opt}}
\end{algorithm}\vspace*{1em}
